Local B-site chemistry controls oxygen-vacancy energetics in Ca-Ce-Ti-Mn perovskites for thermochemical hydrogen production

Two-step thermochemical water splitting driven by concentrated solar heat is a scalable route to renewable hydrogen, but it requires oxides whose oxygen-vacancy formation energies balance facile reduction with favorable reoxidation. Perovskite solid solutions can tune this balance, but the relationship between bulk stoichiometry and local defect energetics remains poorly understood. Here we map oxygen-vacancy formation energetics across Ca-Ce-Ti-Mn (CCTM) perovskites by combining first-principles calculations with a coverage-constrained special quasirandom structure approach that realizes all fifteen symmetry-distinct oxygen nearest-neighbor environments, an interpretable crystal-feature model whose fitted coefficients directly encode the underlying Born-Haber thermochemistry, and a fine-tuned defect graph neural network. Local B-site chemistry dominates the oxygen-vacancy formation energy $E_\mathrm{v}$: varying the nearest-neighbor Mn fraction shifts $E_\mathrm{v}$ by 1.0-1.5 eV depending on local Ce content, whereas A-site Ce variation contributes a smaller, Mn-dependent shift of 0.2-0.6 eV. Short-range B-site cation order, if it can be established and kinetically retained through processing, is therefore a candidate means of tuning redox performance without changing bulk composition. Composition-space maps identify a Ce/Mn-balanced region (~29-33% Ce on the A site and 58-67% Mn on the B site) combining a high fraction of vacancy sites within the targeted $E_\mathrm{v}$ window with phase stability and solubility, whose predicted redox cycle capacity matches or exceeds the ceria benchmark at 1350 $^\circ$C rather than the roughly 1600 $^\circ$C ceria requires. Measurements on three CCTM compositions show cycle capacity increasing monotonically with Ce content under protocols close to the model conditions. The design rules are expected to transfer to related perovskite families.

==> xref-esi.tex <==
% Labels frozen from esi.aux for arXiv (xr cannot run there).
\makeatletter
\newlabel{S-sec:esi:magmoments}{{S1}{1}{}{}{}}
\newlabel{S-sec:esi:magmoments@cref}{{[section][1][]S1}{[1][1][]1}{}{}{}}
\newlabel{S-tbl:esi:ce-counts}{{S1}{2}{}{}{}}
\newlabel{S-tbl:esi:ce-counts@cref}{{[table][1][]S1}{[1][2][]2}{}{}{}}
\newlabel{S-tbl:esi:dmu}{{S2}{2}{}{}{}}
\newlabel{S-tbl:esi:dmu@cref}{{[table][2][]S2}{[1][2][]2}{}{}{}}
\newlabel{S-fgr:esi:magmoments}{{S1}{3}{}{}{}}
\newlabel{S-fgr:esi:magmoments@cref}{{[figure][1][]S1}{[1][2][]3}{}{}{}}
\newlabel{S-sec:esi:dos}{{S2}{3}{}{}{}}
\newlabel{S-sec:esi:dos@cref}{{[section][2][]S2}{[1][2][]3}{}{}{}}
\newlabel{S-fgr:esi:dos}{{S2}{4}{}{}{}}
\newlabel{S-fgr:esi:dos@cref}{{[figure][2][]S2}{[1][3][]4}{}{}{}}
\newlabel{S-sec:esi:cfm-parity}{{S3}{4}{}{}{}}
\newlabel{S-sec:esi:cfm-parity@cref}{{[section][3][]S3}{[1][3][]4}{}{}{}}
\newlabel{S-eqn:cfm}{{S1}{4}{}{}{}}
\newlabel{S-eqn:cfm@cref}{{[equation][1][]S1}{[1][4][]4}{}{}{}}
\newlabel{S-fgr:cfm-parity}{{S3}{6}{}{}{}}
\newlabel{S-fgr:cfm-parity@cref}{{[figure][3][]S3}{[1][5][]6}{}{}{}}
\newlabel{S-sec:esi:vv-electrostatic}{{S4}{6}{}{}{}}
\newlabel{S-sec:esi:vv-electrostatic@cref}{{[section][4][]S4}{[1][5][]6}{}{}{}}
\newlabel{S-eqn:tf-screened}{{S2}{6}{}{}{}}
\newlabel{S-eqn:tf-screened@cref}{{[equation][2][]S2}{[1][6][]6}{}{}{}}
\newlabel{S-tbl:cfm-subsets}{{S3}{7}{}{}{}}
\newlabel{S-tbl:cfm-subsets@cref}{{[table][3][]S3}{[1][5][]7}{}{}{}}
\newlabel{S-eqn:rWS}{{S3}{7}{}{}{}}
\newlabel{S-eqn:rWS@cref}{{[equation][3][]S3}{[1][7][]7}{}{}{}}
\newlabel{S-fgr:esi:vv-electrostatic}{{S4}{8}{}{}{}}
\newlabel{S-fgr:esi:vv-electrostatic@cref}{{[figure][4][]S4}{[1][7][]8}{}{}{}}
\newlabel{S-sec:esi:xrd}{{S5}{8}{}{}{}}
\newlabel{S-sec:esi:xrd@cref}{{[section][5][]S5}{[1][8][]8}{}{}{}}
\newlabel{S-fgr:xrd}{{S5}{9}{}{}{}}
\newlabel{S-fgr:xrd@cref}{{[figure][5][]S5}{[1][9][]9}{}{}{}}
\newlabel{S-sec:esi:tga}{{S6}{9}{}{}{}}
\newlabel{S-sec:esi:tga@cref}{{[section][6][]S6}{[1][9][]9}{}{}{}}
\newlabel{S-fgr:esi:xrd-postcycling}{{S6}{10}{}{}{}}
\newlabel{S-fgr:esi:xrd-postcycling@cref}{{[figure][6][]S6}{[1][9][]10}{}{}{}}
\newlabel{S-fgr:tga}{{S7}{11}{}{}{}}
\newlabel{S-fgr:tga@cref}{{[figure][7][]S7}{[1][10][]11}{}{}{}}
\newlabel{S-sec:esi:thermo}{{S7}{12}{}{}{}}
\newlabel{S-sec:esi:thermo@cref}{{[section][7][]S7}{[1][12][]12}{}{}{}}
\newlabel{S-sec:esi:thermo:derivation}{{S7.1}{12}{}{}{}}
\newlabel{S-sec:esi:thermo:derivation@cref}{{[subsection][1][7]S7.1}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:vac-reaction}{{S4}{12}{}{}{}}
\newlabel{S-eqn:vac-reaction@cref}{{[equation][4][]S4}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:DeltaGv-raw}{{S5}{12}{}{}{}}
\newlabel{S-eqn:DeltaGv-raw@cref}{{[equation][5][]S5}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:muO2-split}{{S6}{12}{}{}{}}
\newlabel{S-eqn:muO2-split@cref}{{[equation][6][]S6}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:DeltamuO2}{{S7}{12}{}{}{}}
\newlabel{S-eqn:DeltamuO2@cref}{{[equation][7][]S7}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:DeltaGv-final}{{S8}{12}{}{}{}}
\newlabel{S-eqn:DeltaGv-final@cref}{{[equation][8][]S8}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:Ev-DFT}{{S9}{12}{}{}{}}
\newlabel{S-eqn:Ev-DFT@cref}{{[equation][9][]S9}{[1][12][]12}{}{}{}}
\newlabel{S-eqn:muO-def}{{S10}{12}{}{}{}}
\newlabel{S-eqn:muO-def@cref}{{[equation][10][]S10}{[1][12][]12}{}{}{}}
\newlabel{S-sec:esi:thermo:occupation}{{S7.2}{13}{}{}{}}
\newlabel{S-sec:esi:thermo:occupation@cref}{{[subsection][2][7]S7.2}{[1][12][]13}{}{}{}}
\newlabel{S-eqn:partition}{{S11}{13}{}{}{}}
\newlabel{S-eqn:partition@cref}{{[equation][11][]S11}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:occupation}{{S12}{13}{}{}{}}
\newlabel{S-eqn:occupation@cref}{{[equation][12][]S12}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:p-binomial}{{S13}{13}{}{}{}}
\newlabel{S-eqn:p-binomial@cref}{{[equation][13][]S13}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:delta-avg}{{S14}{13}{}{}{}}
\newlabel{S-eqn:delta-avg@cref}{{[equation][14][]S14}{[1][13][]13}{}{}{}}
\newlabel{S-sec:esi:thermo:references}{{S7.3}{13}{}{}{}}
\newlabel{S-sec:esi:thermo:references@cref}{{[subsection][3][7]S7.3}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:shomate-Cp}{{S15}{13}{}{}{}}
\newlabel{S-eqn:shomate-Cp@cref}{{[equation][15][]S15}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:shomate-H}{{S16}{13}{}{}{}}
\newlabel{S-eqn:shomate-H@cref}{{[equation][16][]S16}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:shomate-S}{{S17}{13}{}{}{}}
\newlabel{S-eqn:shomate-S@cref}{{[equation][17][]S17}{[1][13][]13}{}{}{}}
\newlabel{S-eqn:G-std}{{S18}{14}{}{}{}}
\newlabel{S-eqn:G-std@cref}{{[equation][18][]S18}{[1][13][]14}{}{}{}}
\newlabel{S-eqn:mu-pressure}{{S19}{14}{}{}{}}
\newlabel{S-eqn:mu-pressure@cref}{{[equation][19][]S19}{[1][14][]14}{}{}{}}
\newlabel{S-tbl:shomate}{{S4}{14}{}{}{}}
\newlabel{S-tbl:shomate@cref}{{[table][4][]S4}{[1][14][]14}{}{}{}}
\newlabel{S-sec:esi:thermo:example}{{S7.4}{14}{}{}{}}
\newlabel{S-sec:esi:thermo:example@cref}{{[subsection][4][7]S7.4}{[1][14][]14}{}{}{}}
\newlabel{S-tbl:esi:cctm2112-env}{{S5}{15}{}{}{}}
\newlabel{S-tbl:esi:cctm2112-env@cref}{{[table][5][]S5}{[1][14][]15}{}{}{}}
\newlabel{S-sec:esi:dgnn}{{S8}{15}{}{}{}}
\newlabel{S-sec:esi:dgnn@cref}{{[section][8][]S8}{[1][15][]15}{}{}{}}
\newlabel{S-sec:esi:dgnn:method}{{S8.1}{15}{}{}{}}
\newlabel{S-sec:esi:dgnn:method@cref}{{[subsection][1][8]S8.1}{[1][15][]15}{}{}{}}
\newlabel{S-sec:esi:dgnn:datasets}{{S8.2}{16}{}{}{}}
\newlabel{S-sec:esi:dgnn:datasets@cref}{{[subsection][2][8]S8.2}{[1][16][]16}{}{}{}}
\newlabel{S-sec:esi:dgnn:screening}{{S8.3}{16}{}{}{}}
\newlabel{S-sec:esi:dgnn:screening@cref}{{[subsection][3][8]S8.3}{[1][16][]16}{}{}{}}
\newlabel{S-sec:esi:dgnn:validation}{{S8.4}{17}{}{}{}}
\newlabel{S-sec:esi:dgnn:validation@cref}{{[subsection][4][8]S8.4}{[1][17][]17}{}{}{}}
\newlabel{S-fgr:esi:dgnn:parity}{{S8}{18}{}{}{}}
\newlabel{S-fgr:esi:dgnn:parity@cref}{{[figure][8][]S8}{[1][17][]18}{}{}{}}
\newlabel{S-fgr:esi:dgnn:vs:cfm:distributions}{{S9}{19}{}{}{}}
\newlabel{S-fgr:esi:dgnn:vs:cfm:distributions@cref}{{[figure][9][]S9}{[1][17][]19}{}{}{}}
\newlabel{S-fgr:esi:dgnn:summary}{{S10}{20}{}{}{}}
\newlabel{S-fgr:esi:dgnn:summary@cref}{{[figure][10][]S10}{[1][18][]20}{}{}{}}
\newlabel{S-sec:esi:sqs-sensitivity}{{S9}{20}{}{}{}}
\newlabel{S-sec:esi:sqs-sensitivity@cref}{{[section][9][]S9}{[1][20][]20}{}{}{}}
\newlabel{S-sec:esi:bz-convergence}{{S10}{21}{}{}{}}
\newlabel{S-sec:esi:bz-convergence@cref}{{[section][10][]S10}{[1][20][]21}{}{}{}}
\newlabel{S-fgr:esi:bz-convergence}{{S11}{22}{}{}{}}
\newlabel{S-fgr:esi:bz-convergence@cref}{{[figure][11][]S11}{[1][21][]22}{}{}{}}
\newlabel{S-sec:esi:atomic-props}{{S11}{22}{}{}{}}
\newlabel{S-sec:esi:atomic-props@cref}{{[section][11][]S11}{[1][22][]22}{}{}{}}
\newlabel{S-eqn:cfm-averaging}{{S20}{22}{}{}{}}
\newlabel{S-eqn:cfm-averaging@cref}{{[equation][20][]S20}{[1][22][]22}{}{}{}}
\newlabel{S-tbl:esi:bond-energies}{{S6}{23}{}{}{}}
\newlabel{S-tbl:esi:bond-energies@cref}{{[table][6][]S6}{[1][22][]23}{}{}{}}
\newlabel{S-tbl:esi:reduction-potentials}{{S7}{23}{}{}{}}
\newlabel{S-tbl:esi:reduction-potentials@cref}{{[table][7][]S7}{[1][22][]23}{}{}{}}
\makeatother


==> xref-main.tex <==
% Labels frozen from main.aux for arXiv (xr cannot run there).
\makeatletter
\newlabel{M-sec:results}{{}{3}{}{}{}}
\newlabel{M-sec:results@cref}{{}{[1][2][]3}{}{}{}}
\newlabel{M-tbl:cctm_compositions}{{1}{4}{}{}{}}
\newlabel{M-tbl:cctm_compositions@cref}{{[table][1][]1}{[1][3][]4}{}{}{}}
\newlabel{M-fgr:1}{{1}{4}{}{}{}}
\newlabel{M-fgr:1@cref}{{[figure][1][]1}{[1][3][]4}{}{}{}}
\newlabel{M-tbl:cctm_ev_stats}{{2}{4}{}{}{}}
\newlabel{M-tbl:cctm_ev_stats@cref}{{[table][2][]2}{[1][3][]4}{}{}{}}
\newlabel{M-fgr:2}{{2}{5}{}{}{}}
\newlabel{M-fgr:2@cref}{{[figure][2][]2}{[1][3][]5}{}{}{}}
\newlabel{M-fgr:3}{{3}{5}{}{}{}}
\newlabel{M-fgr:3@cref}{{[figure][3][]3}{[1][3][]5}{}{}{}}
\newlabel{M-fgr:4}{{4}{6}{}{}{}}
\newlabel{M-fgr:4@cref}{{[figure][4][]4}{[1][3][]6}{}{}{}}
\newlabel{M-sec:results:experimental:validation}{{}{6}{}{}{}}
\newlabel{M-sec:results:experimental:validation@cref}{{}{[1][6][]6}{}{}{}}
\newlabel{M-fgr:5}{{5}{7}{}{}{}}
\newlabel{M-fgr:5@cref}{{[figure][5][]5}{[1][6][]7}{}{}{}}
\newlabel{M-tbl:cctm_delta_delta}{{3}{7}{}{}{}}
\newlabel{M-tbl:cctm_delta_delta@cref}{{[table][3][]3}{[1][6][]7}{}{}{}}
\newlabel{M-fgr:6}{{6}{9}{}{}{}}
\newlabel{M-fgr:6@cref}{{[figure][6][]6}{[1][8][]9}{}{}{}}
\newlabel{M-sec:methods}{{}{11}{}{}{}}
\newlabel{M-sec:methods@cref}{{}{[1][11][]11}{}{}{}}
\newlabel{M-eqn:occupation}{{4}{12}{}{}{}}
\newlabel{M-eqn:occupation@cref}{{[equation][4][]4}{[1][12][]12}{}{}{}}
\newlabel{M-eqn:delta-avg-main}{{5}{12}{}{}{}}
\newlabel{M-eqn:delta-avg-main@cref}{{[equation][5][]5}{[1][12][]12}{}{}{}}
\newlabel{M-eqn:thermal-reduction-muO-split}{{6}{12}{}{}{}}
\newlabel{M-eqn:thermal-reduction-muO-split@cref}{{[equation][6][]6}{[1][12][]12}{}{}{}}
\newlabel{M-eqn:water-splitting-equilibrium}{{7}{12}{}{}{}}
\newlabel{M-eqn:water-splitting-equilibrium@cref}{{[equation][7][]7}{[1][12][]12}{}{}{}}
\newlabel{M-eqn:water-splitting-muO-split}{{8}{12}{}{}{}}
\newlabel{M-eqn:water-splitting-muO-split@cref}{{[equation][8][]8}{[1][12][]12}{}{}{}}
\newlabel{M-sec:experimental-methods}{{}{13}{}{}{}}
\newlabel{M-sec:experimental-methods@cref}{{}{[1][13][]13}{}{}{}}
\newlabel{M-LastPage}{{}{17}{}{}{}}
\makeatother

